Band Together: Untargeted Adversarial Training with Multimodal Coordination against Evasion-based Promotion Attacks

Multimodal recommender systems exploit visual and textual signals to alleviate data sparsity, but this also makes them more vulnerable to evasion-based promotion attacks. Existing defenses are largely limited to single-modal settings and mainly focus on poisoning-based threats, leaving evasion-based threats underexplored. In this work, we first identify a cross-modal gradient mismatch under the multi-user promotion setting, where visual and textual perturbations are optimized in inconsistent directions due to the dominance of distinct user groups. This phenomenon dilutes the attack effectiveness and leads robust training to underestimate worst-case risks. To address this issue, we propose Untargeted Adversarial Training with Multimodal Coordination (UAT-MC). UAT-MC tackles the challenge of unknown targeted items in evasion-based attacks (as opposed to poisoning-based attacks) by treating all items as potential targets, and introduces a gradient alignment mechanism to explicitly correct this mismatch. This design ensures synchronized perturbations across modalities, thereby maximizing adversarial strength for robust training. Extensive experiments demonstrate that UAT-MC significantly improves robustness against promotion attacks while maintaining acceptable recommendation performance under the defense-accuracy trade-off. Code is available at https://github.com/gmXian/UAT-MC.

==> Tables/table_diff_gamma.tex <==
\begin{table*}[htbp]
	\centering
	% \vspace{-5mm}
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		Dataset & {Victim Model} & {$\gamma=$0} & {$\gamma=$0.1} & {$\gamma=$1} & {$\gamma=$10} \\
		\hline
		\multirow{2}{*}{Baby} 
		& VBPR & 394.16\% & 409.31\% & \textbf{475.72}\% & 135.50\% \\
		& MMGCN & 117.95\% & 153.55\% & \textbf{266.54}\% & 47.76\% \\
		\hline
		\multirow{2}{*}{Sports} 
		& VBPR & 18569.53\% & 19095.29\% & \textbf{24118.28}\% & 8456.79\% \\
		& MMGCN & 633.83\% & 718.10\% & \textbf{1114.84}\% & 767.36\% \\
		\hline
		\multirow{2}{*}{Clothing} 
		& VBPR & 3610.26\% & 3705.74\% & \textbf{4450.43}\% & 1270.96\% \\
		& MMGCN & 881.53\% & 1420.72\% & \textbf{7542.34}\% & 4588.74\% \\
		\hline
	\end{tabular}
	% \vspace{-3mm}
	\caption{ $\text{Gain}_{\text{Hit}@50}$ (\%) results under different values of the margin parameter $\gamma$ across three datasets and two victim models in FGSM-based promotion attack. The best attack results are highlighted in bold.}
	\label{Table:diff_gamma}
	
\end{table*}


==> UAT-MC-IJCAI-ECAI-26/Tables/table_defense_result.tex <==


\begin{table*}[!t]

	\begin{center}
		\renewcommand{\arraystretch}{1}
		\tabcolsep=0.12cm
		\resizebox{\textwidth}{!}
		{
			\begin{tabular}{|c|c|c|c|cc|cc|cc|cc|cc|}
				\hline
				\multirow{3}{*}{Dataset} & \multirow{3}{*}{\shortstack{Victim\\Model}} & \multirow{3}{*}{\shortstack{Defense\\Method}} \
				& \multirow{3}{*}{$\text{Hit}_{\text{before}}$} \
				& \multicolumn{4}{c|}{FGSM-based Attack}  
				& \multicolumn{4}{c|}{PGD-based Attack} 
				& \multicolumn{2}{c|}{Recommendation} \\
				\cline{5-14} 
				&    &   &  
				         &  \multicolumn{2}{c|}{$\mathcal{L}_{\text{prom}}$}
				         &  \multicolumn{2}{c|}{$\mathcal{L}_{\text{prom}}+\mathcal{L}_{\text{Align}}$}
				          &  \multicolumn{2}{c|}{$\mathcal{L}_{\text{prom}}$}   
				         &  \multicolumn{2}{c|}{$\mathcal{L}_{\text{prom}}+\mathcal{L}_{\text{Align}}$}  
				         & \multirow{2}{*}{Recall} 
				         &\multirow{2}{*}{NDCG} 
				         \\
				   \cline{5-12} 
				  &    &   &  
				         & \shortstack{$\text{Hit}_{\text{after}}$}   
				         & \shortstack{$\text{Gain}_{\text{Hit}}$}    
				         & \shortstack{$\text{Hit}_{\text{after}}$}   
				         & \shortstack{$\text{Gain}_{\text{Hit}}$}    
				         & \shortstack{$\text{Hit}_{\text{after}}$}   
				         & \shortstack{$\text{Gain}_{\text{Hit}}$}  
				         & \shortstack{$\text{Hit}_{\text{after}}$}   
				         & \shortstack{$\text{Gain}_{\text{Hit}}$}   
				         &  
				         & 
				         \\
				         
				\hline
				\multirow{6}{*}{Baby}
				& \multirow{3}{*}{VBPR}
				  & w/o AT   & 0.667\% & 3.865\% & 479.38\% & 3.908\% & 485.80\% & 4.111\% & 516.15\% & 4.143\% & 520.99\% & 0.0503 & 0.027 \\
				& & UAT        & 0.622\% & 2.381\% & 282.96\% & 2.383\% & 283.41\% & 2.450\% & 294.15\% & 2.451\% & 294.25\% & 0.0484 & 0.0264 \\
				& & UAT-MC     & 0.621\% & 1.515\% & \textbf{143.98}\% & 1.515\% &  \textbf{144.00}\% & 1.544\% &  \textbf{148.65}\% & 1.544\% &  \textbf{148.65}\% & 0.0476 & 0.0253 \\
				\cline{2-14} 
				& \multirow{3}{*}{MMGCN}
				  & w/o AT   & 0.622\% & 1.747\% & 181.03\% & 1.748\% & 181.14\% & 3.399\% & 446.76\% & 3.421\% & 450.30\% & 0.0413 & 0.022 \\
				& & UAT        & 0.472\% & 0.507\% & 7.29\% & 0.508\% & 7.49\% & 0.515\% & 9.12\% & 0.516\% & 9.34\% & 0.0344 & 0.0185 \\
				& & UAT-MC     & 0.479\% & 0.513\% &  \textbf{7.21}\% & 0.514\% &  \textbf{7.47}\% & 0.519\% &  \textbf{8.46}\% & 0.520\% &  \textbf{8.62}\% & 0.0341 & 0.0185 \\
				
				\hline
				
				\multirow{6}{*}{Sports}
				& \multirow{3}{*}{VBPR}
				  & w/o AT   & 0.025\% & 6.547\% & 25722.99\% & 6.586\% & 25876.73\% & 7.253\% & 28506.93\% & 7.279\% & 28610.25\% & 0.0586 & 0.0319 \\
				& & UAT        & 0.025\% & 0.028\% & 13.45\% & 0.028\% & 13.45\% & 0.029\% & 13.73\% & 0.029\% & 13.73\% & 0.0510 & 0.0280 \\
				& & UAT-MC     & 0.024\% & 0.026\% &  \textbf{10.32}\% & 0.026\% &  \textbf{10.32}\% & 0.026\% &  \textbf{10.32}\% & 0.026\% &  \textbf{10.32}\% & 0.0508 & 0.0280 \\
				\cline{2-14} 
				& \multirow{3}{*}{MMGCN}
			   	  & w/o AT   & 0.024\% & 0.266\% & 1024.04\% & 0.268\% & 1033.23\% & 0.572\% & 2315.13\% & 0.581\% & 2352.82\% & 0.0385 & 0.0206 \\
				& & UAT        & 0.035\% & 0.038\% & 7.01\% & 0.039\% & 11.02\% & 0.044\% & 24.45\% & 0.044\% & 25.45\% & 0.0313 & 0.0172 \\
				& & UAT-MC     & 0.034\% & 0.034\% &  \textbf{0.00}\% & 0.037\% &  \textbf{8.44}\% & 0.041\% &  \textbf{19.14}\% & 0.041\% &  \textbf{19.14}\% & 0.0317 & 0.0173 \\
				
				\hline
				
				\multirow{6}{*}{Clothing}
				& \multirow{3}{*}{VBPR}
				  & w/o AT   & 0.036\% & 1.335\% & 3558.26\% & 1.380\% & 3682.09\% & 1.419\% & 3788.87\% & 1.438\% & 3838.61\% & 0.0384 & 0.0211 \\
				& & UAT        & 0.031\% & 0.287\% & 818.66\% & 0.303\% & 869.17\% & 0.306\% & 878.50\% & 0.312\% & 898.38\% & 0.0343 & 0.0189 \\
				& & UAT-MC     & 0.030\% & 0.038\% &  \textbf{26.64}\% & 0.038\% &  \textbf{26.85}\% & 0.038\% &  \textbf{27.70}\% & 0.038\% &  \textbf{27.70}\% & 0.0333 & 0.0184 \\
				\cline{2-14} 
				& \multirow{3}{*}{MMGCN}
				  & w/o AT   & 0.014\% & 1.886\% & 13282.43\% & 1.941\% & 13670.72\% & 9.035\% & 64019.37\% & 9.134\% & 64715.32\% & 0.0239 & 0.0123 \\
				& & UAT        & 0.014\% & 0.025\% & 76.00\% & 0.026\% & 81.78\% & 0.035\% & 148.44\% & 0.036\% & 149.33\% & 0.0221 & 0.0114 \\
				& & UAT-MC     & 0.015\% & 0.019\% &  \textbf{29.44}\% & 0.020\% &  \textbf{33.77}\% & 0.032\% &  \textbf{119.05}\% & 0.032\% &  \textbf{121.65}\% & 0.0221 & 0.0115 \\
			
				\hline
				
			\end{tabular}
		}
		
		
	\end{center}
	% \vspace{-3mm}
		\caption{
		Performance of promotion attacks on two classical models. 
		All reported numbers are averaged results. The best defense results are highlighted in bold.
        (Note: $\text{Gain}_{\text{Hit}@50}$ values are computed using unrounded $\text{Hit}@50$ scores).
	}
	\label{table:defense_result}
	\vspace{-3mm}
\end{table*}








==> UAT-MC-IJCAI-ECAI-26/Tables/table_diff_epsilon.tex <==


\begin{table*}[!t]
	\begin{center}
		\small
		\renewcommand{\arraystretch}{1}
		\tabcolsep=0.12cm
		\footnotesize
		\resizebox{\textwidth}{!}
		{
			\begin{tabular}{|c|c|cccc|cccc|}
				\hline
				% \multirow{3}{*}{Dataset} & Victim Model & \multicolumn{4}{c|}{VBPR}  & 
				
				\multirow{2}{*}{Dataset} & Victim Model & \multicolumn{4}{c|}{VBPR} & \multicolumn{4}{c|}{MMGCN} \\
				\cline{2-10}
			
	
				& {$\epsilon$}   & {\rule{0pt}{2ex}$\epsilon_{a}$}=2.5\%   & {$\epsilon_{a}$}=5\%   & {$\epsilon_{a}$}=7.5\%    & {$\epsilon_{a}$}=10\%   & {$\epsilon_{a}$}=2.5\%   & {$\epsilon_{a}$}=5\%   & {$\epsilon_{a}$}=7.5\%    & {$\epsilon_{a}$}=10\%  \\
				\hline
				\multirow{5}{*}{Baby}
				& w/o AT & 54.25\% & 146.19\% & 288.11\% & 479.38\% & 81.49\% & 152.20\% & 176.08\% & 181.03\% \\
				& {$\epsilon_{d}$}=2.5\%    & 49.33\% & 138.78\% & 270.46\% & 456.33\% & 12.39\% & 21.72\% & 27.69\% & 31.13\% \\
				& {$\epsilon_{d}$}=5\%    & 43.01\% & 122.32\% & 243.43\% & 412.88\% & 5.65\% & 9.30\% & 13.07\% & 15.82\% \\
				& {$\epsilon_{d}$}=7.5\%    & 28.82\% & 73.92\% & 142.97\% & 233.41\% & 3.97\% & 7.37\% & 10.82\% & 12.94\% \\
				& {$\epsilon_{d}$}=10\%      & \textbf{19.38}\% & \textbf{48.45}\% &\textbf{89.52}\% & \textbf{143.98}\% & \textbf{2.42}\% & \textbf{4.32}\% & \textbf{5.83}\% & \textbf{7.21}\% \\
				\cline{1-10} 
				\multirow{5}{*}{Sports}
				& w/o AT & 734.90\% & 4636.57\% & 13506.93\% & 25722.99\% & 201.19\% & 505.93\% & 789.32\% & 1024.04\% \\
				& {$\epsilon_{d}$}=2.5\%    & 277.40\% & 1946.12\% & 6601.83\% & 14000.23\% & 30.33\% & 48.74\% & 51.46\% & 45.19\% \\
				& {$\epsilon_{d}$}=5\%    & 58.84\% & 292.82\% & 954.70\% & 2356.63\% & 16.90\% & 21.90\% & 26.43\% & 27.14\% \\
				& {$\epsilon_{d}$}=7.5\%    & 6.90\% & 14.37\% & 22.13\% & 34.48\% & 7.32\% & 8.87\% & 9.98\% & 10.42\% \\
				& {$\epsilon_{d}$}=10\%      & \textbf{2.36}\% & \textbf{4.72}\% & \textbf{7.37}\% & \textbf{10.32}\% & \textbf{0.00}\% & \textbf{3.91}\% & \textbf{4.53}\% & \textbf{6.38}\% \\
				\cline{1-10} 
				\multirow{5}{*}{Clothing}
				& w/o AT & 121.04\% & 519.48\% & 1508.35\% & 3558.26\% & 1072.07\% & 6460.36\% & 12045.05\% & 13282.43\% \\
				& {$\epsilon_{d}$}=2.5\%    & 79.76\% & 327.66\% & 1004.01\% & 2486.97\% & 128.08\% & 252.71\% & 303.45\% & 305.42\% \\
				& {$\epsilon_{d}$}=5\%    & 33.95\% & 100.20\% & 244.99\% & 522.09\% & 43.98\% & 61.28\% & 68.42\% & 71.80\% \\
				& {$\epsilon_{d}$}=7.5\%    & 13.35\% & 36.23\% & 67.37\% & 123.52\% & 30.04\% & 48.50\% & 51.93\% & 56.22\% \\
				& {$\epsilon_{d}$}=10\%      & \textbf{2.96}\% & \textbf{9.30}\% & \textbf{16.70}\% & \textbf{26.64}\% & \textbf{21.65}\% & \textbf{25.06}\% & \textbf{28.04}\% & \textbf{29.44}\% \\
				\cline{1-10} 
				\hline
				
			\end{tabular}
		}
	\end{center}
	% \vspace{-3mm}
	\caption{
		Comparison of $\text{Gain}_{\text{Hit}@50}$ under different combinations of adversarial training budgets ($\epsilon_d$) and attack budgets ($\epsilon_a$) for FGSM-based promotion attacks \emph{without} gradient alignment. Here, $\epsilon_d$ denotes the perturbation budget used during adversarial training, while $\epsilon_a$ represents the perturbation budget used during promotion attacks. The best defense performance under each setting is highlighted in bold.
	}
	\label{table:diff_epsilons}
	% \vspace{-3mm}
\end{table*}




==> UAT-MC-IJCAI-ECAI-26/Tables/table_diff_epsilon_fgsm_align.tex <==


\begin{table*}[!t]
	\begin{center}
		\small
		\renewcommand{\arraystretch}{1}
		\tabcolsep=0.12cm
		\footnotesize
		\resizebox{\textwidth}{!}
		{
			\begin{tabular}{|c|c|cccc|cccc|}
				\hline
				% \multirow{3}{*}{Dataset} & Victim Model & \multicolumn{4}{c|}{VBPR}  & 
				
				\multirow{2}{*}{Dataset} & Victim Model & \multicolumn{4}{c|}{VBPR} & \multicolumn{4}{c|}{MMGCN} \\
				\cline{2-10}
			
	
				& {$\epsilon$}   & {\rule{0pt}{2ex}$\epsilon_{a}$}=2.5\%   & {$\epsilon_{a}$}=5\%   & {$\epsilon_{a}$}=7.5\%    & {$\epsilon_{a}$}=10\%   & {$\epsilon_{a}$}=2.5\%   & {$\epsilon_{a}$}=5\%   & {$\epsilon_{a}$}=7.5\%    & {$\epsilon_{a}$}=10\%  \\
				\hline
				\multirow{5}{*}{Baby}
				& w/o AT & 54.81\% & 148.29\% & 291.56\% & 485.80\% & 81.68\% & 152.74\% & 176.58\% & 181.14\% \\
				& {$\epsilon_{d}$}=2.5\%    & 49.33\% & 138.78\% & 270.46\% & 456.33\% & 12.55\% & 22.02\% & 28.63\% & 32.24\% \\
				& {$\epsilon_{d}$}=5\%    & 43.01\% & 122.32\% & 243.43\% & 412.92\% & 5.71\% & 9.42\% & 13.21\% & 15.97\% \\
				& {$\epsilon_{d}$}=7.5\%    & 28.82\% & 73.92\% & 142.97\% & 233.41\% & 3.97\% & 7.39\% & 10.85\% & 13.05\% \\
				& {$\epsilon_{d}$}=10\%      & \textbf{19.38}\% & \textbf{48.47}\% & \textbf{89.54}\% & \textbf{144.00}\% & \textbf{2.44}\% & \textbf{4.35}\% & \textbf{5.88}\% & \textbf{7.47}\% \\
				\cline{1-10} 
				\multirow{5}{*}{Sports}
				& w/o AT & 754.29\% \quad & 4737.40\% & 13737.12\% & 25876.73\% & 202.37\% & 512.76\% & 807.12\% & 1033.23\% \\
				& {$\epsilon_{d}$}=2.5\%    & 277.40\% & 1947.26\% & 6602.51\% & 14000.68\% & 31.59\% & 52.30\% & 52.72\% & 56.49\% \\
				& {$\epsilon_{d}$}=5\%    & 60.22\% & 296.96\% & 965.75\% & 2384.53\% & 17.38\% & 30.00\% & 30.48\% & 31.19\% \\
				& {$\epsilon_{d}$}=7.5\%    & 7.18\% & 14.66\% & 23.56\% & 35.34\% & 8.65\% & 11.75\% & 13.75\% & 14.63\% \\
				& {$\epsilon_{d}$}=10\%      & \textbf{2.36}\% & \textbf{4.72}\% & \textbf{7.37}\% & \textbf{10.32}\% & \textbf{4.94}\% & \textbf{6.58}\% & \textbf{7.82}\% & \textbf{8.44}\% \\
				\cline{1-10} 
				\multirow{5}{*}{Clothing}
				& w/o AT & 125.91\% & 534.78\% & 1554.78\% & 3682.09\% & 1091.44\% & 6598.65\% & 12292.34\% & 13670.72\% \\
				& {$\epsilon_{d}$}=2.5\%    & 79.76\% & 327.66\% & 1004.61\% & 2488.58\% & 132.02\% & 263.05\% & 327.59\% & 340.89\% \\
				& {$\epsilon_{d}$}=5\%    & 33.95\% & 100.61\% & 244.99\% & 522.70\% & 47.37\% & 70.30\% & 79.70\% & 80.83\% \\
				& {$\epsilon_{d}$}=7.5\%    & 13.35\% & 36.23\% & 67.58\% & 123.73\% & 32.19\% & 54.94\% & 57.08\% & 63.52\% \\
				& {$\epsilon_{d}$}=10\%      & \textbf{3.38}\% & \textbf{9.51}\% & \textbf{16.70}\% & \textbf{26.85}\% & \textbf{22.51}\% & \textbf{27.05}\% & \textbf{29.53}\% & \textbf{33.77}\% \\
				\cline{1-10} 
				\hline
				
			\end{tabular}
		}
	\end{center}
	% \vspace{-3mm}
	\caption{
		Comparison of $\text{Gain}_{\text{Hit}@50}$ under different combinations of adversarial training budgets ($\epsilon_d$) and attack budgets ($\epsilon_a$) for FGSM-based promotion attacks \emph{with} the gradient alignment loss $\mathcal{L}_{\text{Align}}$. Here, $\epsilon_d$ denotes the perturbation budget used during adversarial training, while $\epsilon_a$ represents the perturbation budget used during promotion attacks. A larger value of $\text{Gain}_{\text{Hit}@50}$ indicates higher attack effectiveness and thus weaker defense capability. The best defense performance under each setting is highlighted in bold.
	}
	\label{table:diff_epsilons_fgsm_align}
	% \vspace{-3mm}
\end{table*}




==> UAT-MC-IJCAI-ECAI-26/Tables/table_diff_gamma.tex <==
\begin{table*}[htbp]
	\centering
	% \vspace{-5mm}
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		Dataset & {Victim Model} & {$\gamma=$0} & {$\gamma=$0.1} & {$\gamma=$1} & {$\gamma=$10} \\
		\hline
		\multirow{2}{*}{Baby} 
		& VBPR & 394.16\% & 409.31\% & \textbf{475.72}\% & 135.50\% \\
		& MMGCN & 117.95\% & 153.55\% & \textbf{266.54}\% & 47.76\% \\
		\hline
		\multirow{2}{*}{Sports} 
		& VBPR & 18569.53\% & 19095.29\% & \textbf{24118.28}\% & 8456.79\% \\
		& MMGCN & 633.83\% & 718.10\% & \textbf{1114.84}\% & 767.36\% \\
		\hline
		\multirow{2}{*}{Clothing} 
		& VBPR & 3610.26\% & 3705.74\% & \textbf{4450.43}\% & 1270.96\% \\
		& MMGCN & 881.53\% & 1420.72\% & \textbf{7542.34}\% & 4588.74\% \\
		\hline
	\end{tabular}
	% \vspace{-3mm}
	\caption{ $\text{Gain}_{\text{Hit}@50}$ (\%) results under different values of the margin parameter $\gamma$ across three datasets and two victim models in FGSM-based promotion attack. The best attack results are highlighted in bold.}
	\label{Table:diff_gamma}
	
\end{table*}


==> UAT-MC-IJCAI-ECAI-26/Tables/tables_rs_hyperparameter_search_space.tex <==
% \begin{table}[htbp]
% 	\centering
% 	\begin{tabular}{|c|c|c|}
% 		\hline
% 		\textbf{Model} & \textbf{Non-shared} & \textbf{Shared} \\
% 		\hline
% 		\multirow{4}{*}{VBPR} 
% 		& &\multirow{9}{*}{
% 			\begin{tabular}[t]{@{}l@{}}
% 				embedding-size=64 \\
% 				epochs $\in [1,1000]$ \\
% 				stopping-step= $100$ \\
% 				train batch size: $2048$ \\
% 				learner: Adam \\
% 				learning rate scheduler $\in[1.0, 50]$ \\
% 				eval batch size=$4096$\\
% 				align-weight $\in \{2.0,1.0,1e-01, 1e-02,1e-3,0\}$
% 			\end{tabular}
% 		} \\
% 		& $\beta \in \{2.0, 1.0, 1e-01, 1e-02,$  & \\
% 		& $1e-03, 1e-04, 1e-05\}$  & \\
% 		& learning-rate= $0.001$ & \\
		
% 		\cline{1-2} 
		
% 		\multirow{6}{*}{MMGCN} 
% 		& & \\
% 		& $\beta \in $: $\{0.00001, 0.0001, 0.001, 0.01, 0.1, 0.5\}$ & \\
% 		& n-layers= $2$ & \\
% 		& learning-rate $\in \{0.0001, 0.0005, 0.001, 0.005, 0.01\}$ & \\
% 		& & \\
% 		& & \\
% 		\hline
% 	\end{tabular}
% 	\caption{Hyper-parameter search spaces of multimodal recommendation systems}
% 	\label{Table:hyper_parameter}
% \end{table}
\begin{table}[t]
    \centering
    \small 
    \renewcommand{\arraystretch}{1.2} 
    \setlength{\tabcolsep}{4pt}
    
    \begin{tabular}{l p{0.65\columnwidth}}
        \toprule
        \textbf{Hyperparameter} & \textbf{Value / Search Space} \\
        \midrule
        \multicolumn{2}{c}{\textit{Common Settings (Shared)}} \\
        \midrule
        Embedding Size & $64$ \\
        Epochs & $[1, 1000]$ \\
        Stopping Step & $100$ \\
        Batch Size & $2048$ (Train), $4096$ (Eval) \\
        Optimizer & Adam \\
        LR Scheduler & $[1.0, 50]$ \\
        Align Weight & $\{2.0, 1.0, 0.1, 0.01, 0.001, 0\}$ \\
        \midrule
        \multicolumn{2}{c}{\textit{VBPR Specific}} \\
        \midrule
        Learning Rate & $0.001$ \\
        $\beta$ & $\{2.0, 1.0, 0.1, 0.01, 0.001, 10^{-4}, 10^{-5}\}$ \\
        \midrule
        \multicolumn{2}{c}{\textit{MMGCN Specific}} \\
        \midrule
        Layers & $2$ \\
        Learning Rate & $\{0.0001, 0.0005, 0.001, 0.005, 0.01\}$ \\
        $\beta$ & $\{10^{-5}, 10^{-4}, 0.001, 0.01, 0.1, 0.5\}$ \\
        \bottomrule
    \end{tabular}
    \caption{Hyper-parameter search spaces of multimodal recommendation systems.}
    % \vspace{-1em}
    \label{Table:hyper_parameter}
\end{table}
